Optimal binary gratings for multi-wavelength magneto-optical traps

Grating magneto-optical traps are an enabling quantum technology for portable metrological devices with ultracold atoms. However, beam diffraction efficiency and angle are affected by wavelength, creating a single-optic design challenge for laser cooling in two stages at two distinct wavelengths - as commonly used for loading e.g. Sr or Yb atoms into optical lattice or tweezer clocks. Here, we optically characterize a wide variety of binary gratings at different wavelengths to find a simple empirical fit to experimental grating diffraction efficiency data in terms of dimensionless etch depth and period for various duty cycles. The model avoids complex 3D light-grating surface calculations, yet still yields results accurate to a few percent across a broad range of parameters. Gratings optimized for two (or more) wavelengths can now be designed in an informed manner suitable for a wide class of atomic species enabling advanced quantum technologies.

==> missing <==
@misc{MaxwellCode,
author = "", 
journal="Code is available through e.g. {\href{https://meep.readthedocs.io/en/latest/}{MEEP}},  {\href{https://pages.nist.gov/pySCATMECH/index.html}{pySCATMECH} (open source), or \href{https://www.lumerical.com/}{Lumerical}}"}
